Decomposition and factorisation of transients in Functional Graphs

Functional graphs (FGs) model the graph structures used to analyse the behaviour of functions from a discrete set to itself. In turn, such functions are used to study real complex phenomena evolving in time. As the systems involved can be quite large, it is interesting to decompose and factorise them into several subgraphs acting together. Polynomial equations over functional graphs provide a formal way to represent this decomposition and factorisation mechanism, and solving them validates or invalidates hypotheses on their decomposability. The current solution method breaks down a single equation into a series of basic equations of the form AxX = B (with A, X, and B being FGs) to identify the possible solutions. However, it is able to consider just FGs made of cycles only. This work proposes an algorithm for solving these basic equations for general connected FGs. By exploiting a connection with the cancellation problem, we prove that the upper bound to the number of solutions is closely related to the size of the cycle in the coefficient A of the equation. The cancellation problem is also involved in the main algorithms provided by the paper. We introduce a polynomial-time semi-decision algorithm able to provide constraints that a potential solution will have to satisfy if it exists. Then, exploiting the ideas introduced in the first algorithm, we introduce a second exponential-time algorithm capable of finding all solutions by integrating several 'hacks' that try to keep the exponential as tight as possible.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
A Finite Discrete Dynamical System (DDS) $\dds=\structure{\setst,f}$ consists of a finite set of states $\setst$ and a \emph{next-state map} $f:\setst\to\setst$, which defines a successor for each state of $\setst$.
A DDS can also be represented by a digraph, called the \emph{dynamics graph}, where the vertices are the possible states of the system, and the function $f$ defines the existing edges (thus nodes have outgoing degree equal to $1$). 
Since $\setst$ is finite, each state $s\in\setst$ is \emph{ultimately periodic} \ie each long enough path originating in $s$ will eventually run into a cycle. Hence, nodes of a dynamics graph can be classified as \emph{periodic} if they belong to a cycle, and \emph{transient} otherwise. 
From a mathematical point of view, DDS are a simple model, but they find important applications in the modelling of many real-world phenomena, namely, Boolean automata networks, genetic regulatory networks, cellular automata, and many others \cite{Sene12, bower2004computational, AlonsoSanz12}.  In the literature, many studies are concerned with the computational complexity of problems over DDS \cite{barrett2000b,barret2001,barret2001b,BARRETT2006,FormentiMP14,DennunzioFMP19,BridouxGPS21,BridouxDPR22}. 
Computational complexity is an issue here since the interesting questions for the applications have, most of the times, high computational complexity. A research direction, developed recently, tries to control this complexity by splitting the main the DDS under study into simpler ones by adopting a suitable algebraic approach. Indeed, it has been proved that DDS equipped with sum (\ie disjoint union of components) and product operations (\ie direct product of graphs) forms a commutative semiring~\cite{dorigatti2018, weichsel1962kronecker}. Thanks to this algebraic setting, one can write polynomial equations in which coefficients and unknowns are DDS. Then, to simplify a certain DDS, one needs to solve a polynomial equation having the DDS as its constant right-hand side. If a solution exists, it can be combined with the coefficients of the equation in order to obtain the original dynamics by means of smaller DDS.
To solve these equations, one needs to be able to solve a finite number of basic linear equation of the form $A \cdot X=B$, where $A$ and $B$ are known DDS and $X$ is unknown~\cite{dennunzio2019solving}. To the best of our knowledge, a technique has been introduced to solve these equations, and more general ones, just over DDS without transient states~\cite{dennunzio2019solving, formenti2021mdds}. 

For this reason, this work aims to study equations $A \cdot X=B$ over arbitrary connected DDS $A$, $X$, and $B$ including transient states. 

The idea is to exploit the connection with the classical \emph{cancellation problem} on graphs which aims at establishing under which conditions the isomorphism of $A\diamond X$ and $A\diamond Y$ implies that $X$ and $Y$ are isomorphic, for a graph product $\diamond$~\cite{hammack2011handbook}. The cancellation problem has been investigated over Cartesian, strong, and direct products over different classes of graphs (oriented and not oriented, as well as, admitting self-loops or not)~\cite{lovasz1971cancellation, hammack2009direct, hammack2011handbook}. From the literature, we know that cancellation holds, under certain conditions, for the Cartesian and the strong products (over graphs and digraphs), but it can fail for the direct product. Moreover, it is known that this problem is more challenging over digraphs than over graphs. Some questions are still open concerning the cancellation problem for the direct product over digraphs. Some works have been done to characterise \emph{zero divisors} (digraphs for which the cancellation fails), or to find all digraphs $Y$ such that $A \cdot X=A \cdot Y$, with $A$ and $X$ fixed~\cite{hammack2014zero}. All these works have been done considering generic digraphs. In this work, we want to benefit from the fact that the DDS considered are connected digraphs with outgoing degree one.

We show that cancellation holds over structures suitable for modelling DDS, namely  
infinite in-trees (Theorem~\ref{th:isoinfinitetree}). 
This will allow us to prove an upper-bound for the number of solutions of basic linear equations (Theorem~\ref{upperbound}). This result is important since it allows us to conceive a polynomial time algorithm (Sec.~\ref{poly}) which 1) provides precise constraints on potential solutions 2) discards impossible equations when it is not possible to determine those constraints.
The ideas and results of the first algorithm are
improved and extended to obtain a second one which provides all $X$ of basic equations
(Sec.~\ref{exp}) in exponential time.

Finally, the performances of the second algorithm are evaluated through experiments.
\medskip

Remark that for lack of space, most of the proofs, some example and the pseudo-code of Algorithm $1$ have been moved to the appendix.
%In Section \ref{notation}, we will introduce the abstraction chosen to represent the dynamics of $A$, $X$, and $B$.  Then, in Section \ref{cancellation}, we will show under which conditions cancellation holds over infinite in-trees (able to model the dynamics of DDS), and we will use it to introduce an upper bound to the number of solutions for the basic equation over DDS. By exploiting this result, we will introduce two different algorithms. First, in Section \ref{poly}, we introduce a polynomial time algorithm that can give some information about the possible solutions of the equation over DDS, if at least a solution exists. This also allows us to efficiently detect some impossible equations. In fact, we are sure that the basic equation over DDS is impossible if this algorithm cannot find a solution. Then, we modify the algorithm to obtain an exponential time version that can give all possible values of $X$. This version, presented in Section \ref{exp}, is also based on a useful representation of the transient parts of DDS, but it exploits some properties of the direct product of dynamics graphs and a backtrack mechanism to find all $X$. Thanks to these ideas, we limit the combinatorial explosion of the problem, and the algorithm shows good performance in solving basic equations over DDS. 


==> tikzlibraryoodgraph.code.tex <==
%
% OODGraph: One Out-Degree Graphs library
%
% This library draws connected graphs with out-degree one. To draw unconnected OOD graphs, just draw separatedly their connected components
%
%\RequirePackage{etoolbox}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% This code below have been borrowed from etoolbox package  ----|          %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%V% % % %
\newcommand*{\oodgraph@csxdef}[2]{\expandafter\xdef\csname#1\endcsname{#2}}
\newcommand*{\oodgraph@ifcsdef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\newcommand*{\oodgraph@ifcsundef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}
\newcommand*{\oodgraph@csuse}[1]{%
  \ifcsname#1\endcsname
    \csname#1\expandafter\endcsname
  \fi}
\newcommand{\oodgraph@cslet}[2]{%
    \expandafter\let\csname#1\endcsname#2}
\newcommand*{\oodgraph@csgundef}[1]{\global\oodgraph@cslet{#1}\relax}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % A %
% The above code have been borrowed from etoolbox package  ----| %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%
% Version 0.1 (2019/05/25):
% - first public release
% Version 0.2 (2019/06/01):
% - added /.store in key
% - added /.default key
% - cleaned up code
% Version 0.3 (2019/06/14)
% - fixed drawing algorithm
% - points definitions are now saved in a list
% - the points list is emptied at the closing of the environment oodgraph
% Version 0.4 (2019/06/18)
% - now commands are completely scoped
% - redisigned the graph printing algorithm to take into account that now
%    everything is scoped
% Version 0.45 (2019/06/19)
% - added the option 'rotation angle'
% Version 0.46 (2019/06/20)
% - added the option 'node content'
% - added bridge to tikz and pgf when a key is not known
% - made the library independent of 'etoolbox' package (borrow
%    some code from the package)
% - added oodgraph@ prefix to all commands so to avoid conflicts with other
%    packages/libraries
% Version 0.47 (2019/06/28)
% - options 'oodgraph arrow' and 'oodgraph node' renamed into 'oodgraph edges' and 'oodgraph nodes' for more consistancy
% - fixed a bug with edges style
% - now '->' is the default edge style
% Version 0.48 (2019/07/14)
% - added a check in \addorigin to verifiy if the point has been defined before
% - some code polishing (eliminated the list oodgraph@more@options which is no
%    more used, deleted \oodgraph@resetkeys function and integrated its code
%    directly into the calling functions since its body contained only an \end{scope}
%    command, deleted several unuseful \expandafter commands)
% - explicited the definition of oodgraph@csxdef
% - partially rewritten the drawing routine for beards. Now it is much faster
% Version 0.50 (2019/07/15)
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - introduced the option 'loop style' which allows to style the loops
% - fixed a bug for the special case of cycles of order 2 which drawn the two edges
%   one over the other (obtening a double arrow). Thanks to François Doré for signalling
%   this.
% - bug fix: the beards to be wrongly oriented when the xshift key
%   was used in the addcycle command. Bug discovery and fix by François Doré
% - bug fix: when a cycle had only 2 nodes, they addresses where exchanged. Thanks
%   to François Doré for signalling this

\def\fileversion{0.50}
\def\filedate{2019/08/21}
\message{Library OODGraph}
\message{ v.\ \fileversion, \filedate}
% load tikz dependencies
\usetikzlibrary{calc}
\makeatletter
\gdef\oodgraph@tmp{}
\gdef\oodgraph@points@list{}
%
% convenience routines to extract the prefix from a node path
%
\def\oodgraph@get@prefix@from@path@@#1-#2\pgf@eov{\xdef\oodgraph@tmp{\oodgraph@csuse{#1.origin}}}
\def\oodgraph@get@prefix@from@path#1{
\pgfutil@in@{-}{#1}
\ifpgfutil@in@% if there is a minus sign then it is a package defined point
\oodgraph@get@prefix@from@path@@#1\pgf@eov
\else% regular pgf/tikz point
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\xdef\oodgraph@tmp{(\XCoord,\YCoord)}
\fi
}
%
%  oodgraph@addtolist
%  #1 = name of the list to add to
%  #2 = object to be added
% Service function to append objects to lists
%
\newcommand*{\oodgraph@addtolist}[2]{%
   \expandafter\if\expandafter\relax\csname #1\endcsname\relax%
      \expandafter\expandafter\xdef\csname #1\endcsname{#2}%
   \else%
    \expandafter\xdef\csname #1\endcsname{\csname #1\endcsname,#2}%
\fi%
}
%
%  oodgraph@docslist@undeft
%  #1 = separator char
%  #2 = name of the list
% Service routine to \csundef all elements of the list
% 
\newcommand{\oodgraph@docslist@undef}[2][,]{%
%   #1 = separation char
%   #2 = list
   \def\dolist##1{\expandafter\@dolist##1#1\@eol}%
   \def\@dolist##1#1##2\@eol{%
   % process stuff here with ##1
   \oodgraph@csgundef{##1}
   \ifx\@eol##2\@eol\else\@dolist##2\@eol\fi}%
   \dolist{#2}%
}
%
\pgfkeys{/oodgraph/.search also={/tikz, /pgf}} %,/oodgraph/catch unknown}}%
%\pgfkeys{/oodgraph/.search also={/tikz,/pgf,/oodgraph/catch unknown}}%
\pgfkeys{%
/oodgraph/.cd,
%radius/.initial={1},
radius/.value required,
radius/.default={1},
radius/.store in=\oodgraph@radius,
radius,
%attach node/.initial={a->1},
attach node/.value required,
attach node/.default={a->1},
attach node/.store in=\oodgraph@attach@node,
attach node,
%nodes prefix/.initial={a},
nodes prefix/.value required,
nodes prefix/.default={a},
nodes prefix/.store in=\oodgraph@nodes@prefix,
nodes prefix,
%opening angle/.initial={120},
opening angle/.value required,
opening angle/.default={120},
opening angle/.store in=\oodgraph@opa,
opening angle,
rotation angle/.value required,
rotation angle/.default={0},
rotation angle/.store in=\oodgraph@rota,
rotation angle,
nodes content/.value required,
nodes content/.default={$\bullet$},
nodes content/.store in=\oodgraph@node@content,
nodes content,
nodes@style/.style={},
edges@style/.style={->},
loop@style/.style={out=-30, in=-150,looseness=6},
nodes style/.code=\pgfkeys{/oodgraph/nodes@style/.style={#1}},
edges style/.code=\pgfkeys{/oodgraph/edges@style/.style={#1}},
loop style/.code=\pgfkeys{/oodgraph/loop@style/.style={#1}},
semi thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={semi thick}},
thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={thick}},
ultra thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={ultra thick}},
edges color/.code=\pgfkeys{/oodgraph/edges@style/.append style={#1}},
nodes color/.code=\pgfkeys{/oodgraph/nodes@style/.append style={#1}},
}
%\pgfkeys{/oodgraph/.unknown/.code={%
%\ifx#1\pgfutil@empty\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname}\else\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname=#1}
%\fi}}
%
\newenvironment{oodgraph}[1][]{\begin{scope}[#1]}
{% closing the environment
% free all points definition in the current list
%\forcsvlist{\csgundef}{\oodgraph@points@list}
\expandafter\oodgraph@docslist@undef\expandafter{\oodgraph@points@list}
% free the points list
\gdef\oodgraph@points@list{}
% free temporary definitions
\gdef\oodgraph@tmp{}
\end{scope}}
%
\newcommand{\oodgraph@processkeys}[1][]{
\begin{scope}
\pgfkeys{/oodgraph/.cd,#1}
}
\long\def\oodgraph@drawcycle#1;{
\ifnum#1=1\oodgraph@drawcycle@\else%
{\ifnum#1=2\oodgraph@drawcycle@@{#1}\else%
\oodgraph@drawcycle@@@{#1}\fi}\fi%
% record circle center on points list and define it
\path(0,0);\pgfgetlastxy{\XCoord}{\YCoord};%
\oodgraph@ifcsundef{\oodgraph@nodes@prefix.origin}{%
% if undefined then add to the point list
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix.origin}%
}%
{% if already defined then simply replace the old definition
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
}%
\end{scope}
}
%
\newcommand{\oodgraph@drawcycle@}{
%\pgfcoordinate{myorigin}{\pgfpointorigin}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at(0,0){\oodgraph@node@content};
% save points on the list
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
%\expandafter\oodgraph@csxdef\expandafter{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/loop@style] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@}{
% second node
\pgfmathsetmacro{\oodgraph@half@radius}{.5*\oodgraph@radius}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->2) at(-\oodgraph@half@radius,0){\oodgraph@node@content};
% first node
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at(\oodgraph@half@radius,0){\oodgraph@node@content};
% register nodes
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->2}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(-\oodgraph@half@radius,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->2}{(\oodgraph@half@radius,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/edges@style, bend left] (\oodgraph@nodes@prefix->2);
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->2) edge[/oodgraph/edges@style, bend left] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@@}[1]{
\pgfmathsetmacro\myangle{360.0/#1}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\curangle{(\i-1)*\myangle}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->\i) at ({\oodgraph@radius*cos(\curangle)},{\oodgraph@radius*sin(\curangle)}){\oodgraph@node@content};
  \path(\oodgraph@nodes@prefix->\i); \pgfgetlastxy{\XCoord}{\YCoord};
  \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->\i}
  \oodgraph@csxdef{\oodgraph@nodes@prefix->\i}{(\XCoord,\YCoord)}
}
%\wlog{list=\oodgraph@points@list}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\mynext{ifthenelse(\i==#1,int(1),int(\i+1))}
  \draw[/oodgraph/edges@style] (\oodgraph@nodes@prefix->\i) -- (\oodgraph@nodes@prefix->\mynext);
}
}
\newcommand*{\addcycle}[1][]{%
\oodgraph@processkeys[#1]%
\oodgraph@drawcycle%
}
%
\def\addorigin#1;{%
\pgfutil@ifundefined{pgf@sh@ns@#1}{
\edef\mymsgtmp{No point named #1\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the point has been correctly defined via the standard TikZ interface.}
}{%
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{#1}{(\XCoord,\YCoord)}%
\oodgraph@csxdef{#1.origin}{(\XCoord,\YCoord)}%
%\oodgraph@addtolist{oodgraph@points@list}{#1} % added v. 0.48
%\oodgraph@addtolist{oodgraph@points@list}{#1.origin} % added v. 0.48
}}
%
\newcommand{\addbeard}[1][]{%
\oodgraph@processkeys[#1]
\oodgraph@drawbeardlev
}
\def\oodgraph@drawbeardlev#1;{%
%\wlog{list=\oodgraph@points@list}
\ifnum#1=1\oodgraph@drawbeardlev@\else\oodgraph@drawbeardlev@@{#1}\fi
\end{scope}}
\newcommand{\oodgraph@drawbeardlev@}{
\oodgraph@ifcsdef{\oodgraph@attach@node}{%
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
%\path[reset cm]\oodgraph@csuse{\oodgraph@attach@node};\pgfgetlastxy{\XCoord}{\YCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}{% else signal errors
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists
a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% recompute the coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\myalphatmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\myalpha{ifthenelse(\XCoord>=0,\myalphatmp,180+\myalphatmp)}
\pgfmathsetmacro\myalpha{\myalpha+\oodgraph@rota}
%
% draw the new node
\node[/oodgraph/nodes@style](\oodgraph@attach@node->1) at ($(\oodgraph@attach@node)+({\oodgraph@radius*cos(\myalpha)},{\oodgraph@radius*sin(\myalpha)})$){\oodgraph@node@content};
\draw[/oodgraph/edges@style] (\oodgraph@attach@node->1) -- (\oodgraph@attach@node);
% store infos about node
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->1}
\path(\oodgraph@attach@node->1); \pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{\oodgraph@attach@node->1}{(\XCoord,\YCoord)}
\end{scope}
}
\newcommand{\oodgraph@drawbeardlev@@}[1]{
% #1= number of nodes in the level
% check if the attachment node has been previously defined
\oodgraph@ifcsdef{\oodgraph@attach@node}{% then part
% if the attach node has been defined then
% find the root prefix and retrive the origin
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}% end of then part
{% if it is not defined, print an error message
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% myangle = angle between two successive points of the beard level
\pgfmathsetmacro\myangle{\oodgraph@opa/#1}
% recompute coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\myalphatmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\myalpha{ifthenelse(\XCoord>=0,\myalphatmp,180+\myalphatmp)}
\pgfmathsetmacro\myalpha{\myalpha+\oodgraph@rota}
% compute the offset angle
\pgfmathsetmacro\myofsangle{ifthenelse(mod(#1,2)==1,0.0,\myangle/2.0}
% draw nodes and edges
%\node at (6,6.5){alpha corr=\myalphacorr};
%\node at (6,6){\oodgraph@attach@node=\csuse{\oodgraph@attach@node}};
%\node at (6,5){point=(\XCoord,\YCoord)};
%\node at (6,4.5){myalpha=\myalpha};
%\node at (6,4.5){myangle=\myangle};
%\node at (6,4){myofsangle=\myofsangle};
%\node at (6,3.5){myend=\myend};
\pgfmathsetmacro\myend{int(ceil(#1/2.0))}
\pgfmathsetmacro\myalpha{\myalpha+\myend*\myangle+2*\myofsangle}
\foreach \i in {#1,...,1}{
\pgfmathsetmacro\mycurangle{\myalpha-(#1-\i+1)*\myangle-\myofsangle}
%\node at (6,3.5-\i){mycurangle=\mycurangle};
\node[/oodgraph/nodes@style](\oodgraph@attach@node->\i) at ($(\oodgraph@attach@node)+({\oodgraph@radius*cos(\mycurangle)},{\oodgraph@radius*sin(\mycurangle)})$){\oodgraph@node@content};
  \draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- (\oodgraph@attach@node);
  % save points to points@list
  \path(\oodgraph@attach@node->\i); \pgfgetlastxy{\XCoord}{\YCoord};
 \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->\i}
 \oodgraph@csxdef{\oodgraph@attach@node->\i}{(\XCoord,\YCoord)}
}
\end{scope}}
%
\makeatother
%
\endinput
